On Gossip Algorithms for Machine Learning with Pairwise Objectives

In the IoT era, information is more and more frequently picked up by connected smart sensors with increasing, though limited, storage, communication and computation abilities. Whether due to privacy constraints or to the structure of the distributed system, the development of statistical learning methods dedicated to data that are shared over a network is now a major issue. Gossip-based algorithms have been developed for the purpose of solving a wide variety of statistical learning tasks, ranging from data aggregation over sensor networks to decentralized multi-agent optimization. Whereas the vast majority of contributions consider situations where the function to be estimated or optimized is a basic average of individual observations, it is the goal of this article to investigate the case where the latter is of pairwise nature, taking the form of a U -statistic of degree two. Motivated by various problems such as similarity learning, ranking or clustering for instance, we revisit gossip algorithms specifically designed for pairwise objective functions and provide a comprehensive theoretical framework for their convergence. This analysis fills a gap in the literature by establishing conditions under which these methods succeed, and by identifying the graph properties that critically affect their efficiency. In particular, a refined analysis of the convergence upper and lower bounds is performed.

==> additional_experiments.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{.45\columnwidth}
    \includegraphics[width=\columnwidth]{async_ml_standard}
    \caption{Evolution of the objective function and its standard deviation (asynchronous setting)}\label{fig:async_ml_standard}
  \end{subfigure}
  \begin{subfigure}[t]{.45\columnwidth}
    \includegraphics[width=\columnwidth]{async_ml_bias}
    \caption{Evolution of the bias term}
    \label{fig:async_ml_bias}
  \end{subfigure}
  % \caption{Metric learning: evolution of the bias term $\overline{\epsilon}^n(t)^{\top}\omega(t)$.}
  \caption{Metric learning experiments.}
\end{figure*}

\section{Metric Learning}
We now turn to a metric learning application. We consider the family of Mahalanobis distances $D_{\boldsymbol{\theta}}(\mathbf{x}_i,\mathbf{x}_j) = (\mathbf{x}_i - \mathbf{x}_j)^{\top} \boldsymbol{\theta} (\mathbf{x}_i - \mathbf{x}_j)$ parameterized by $\boldsymbol{\theta}\in\mathbb{S}_+^d$, where $\mathbb{S}_+^d$ is the cone of $d\times d$ positive semi-definite real-valued matrices.
Given a set of data points $\mathbf{x}_1, \dots, \mathbf{x}_n\in\bbR^d$ with associated labels $\ell_1,\dots,\ell_n\in\{-1,1\}$, the goal is to find $\boldsymbol{\theta}\in\mathbb{S}_+^d$ which minimizes the following criterion \citep{jin2009a}:
$$R_n(\boldsymbol{\theta}) = \frac{1}{n^2} \sum_{1 \leq i, j \leq n} \big[\ell_i \ell_j (b - D_{\boldsymbol{\theta}}(\mathbf{x}_i, \mathbf{x}_j)) \big]_+ + \psi(\boldsymbol{\theta}),$$
% where $[u]_+=\max(0,1-u)$ and $b > 0$. As done in the literature, we restrict our attention to Mahalanobis distances parameterized by $\boldsymbol{\theta}\in\mathbb{S}_+^d$, where $\mathbb{S}_+^d$ is the cone of $d\times d$ positive semi-definite real-valued matrices:
% \[
%   R(\boldsymbol{\theta}) = \frac{1}{n^2} \sum_{1 \leq i, j \leq n} \big(\ell_i \ell_j (b - (\mathbf{x}_i - \mathbf{x}_j)^{\top} \boldsymbol{\theta} (\mathbf{x}_i - \mathbf{x}_j)) \big)_+,
% \]
where $[u]_+=\max(0,1-u)$, $b > 0$, and $\psi(\boldsymbol{\theta})=\infty$ if $\boldsymbol{\theta}\notin\mathbb{S}_+^d$ and $0$ otherwise.
We use a synthetic dataset of $n=1,000$ points generated as follows: each point is drawn from a mixture of $10$ Gaussians in $\mathbb{R}^{40}$ (each corresponding to a class) with all Gaussian means contained in a 5d subspace and their shared covariance matrix proportional to the identity with a variance factor such that some overlap is observed. %That is, the solution to the metric learning problem should be proportional to the linear projection over the subspace containing the gaussians means.

Figure~\ref{fig:async_ml_standard} shows the evolution of the objective function and its standard deviation for the asynchronous setting. As in the case of AUC maximization, the algorithm converges much faster on the well-connected networks than on the cycle network. Again, we can see in Figure~\ref{fig:async_ml_bias} that the bias vanishes very quickly with the number of iterations.

We also compare the logistic loss associated to our algorithm's iterates to the loss associated to the following baseline: instead of adding the biased estimate $\nabla f(\boldsymbol{\theta}_i(t); \mathbf{x}_i, \mathbf{y}_i(t))$ to its dual variable $\mathbf{z}_i(t)$, a node $i \in [n]$ receives a vector drawn uniformly at random from the set of gradients $\{ \nabla f(\boldsymbol{\theta}_i(t); \mathbf{x}_i, \mathbf{x}_1), \ldots, \nabla f(\boldsymbol{\theta}_i(t); \mathbf{x}_i, \mathbf{x}_n) \}$. The bias introduced by the random walk procedure is already shown to be very small in comparison to the objective function on Figure~\ref{fig:async_ml_bias}. Here, Figure~\ref{fig:async_ml_baseline-vs-gossip} evidences the fact that this small bias has close to no influence on the optimization process for well-connected networks.

Finally, we focus on decentralized metric learning on the Breast Cancer Wisconsin Dataset. Figure~\ref{fig:async_ml_cancer_standard} shows the evolution of the metric learning criterion with the number of iterations, averaged over $50$ runs. As in previous experiments, there is almost no difference between the convergence rate of the Watts-Strogatz network and the complete network. Moreover, the bias term is again largely negligible when compared to the metric learning criterion, as shown on Figure~\ref{fig:async_ml_cancer_bias}.

\begin{figure}[t]
  \centering
  \includegraphics[width=.9\textwidth]{./images/async_ml_baseline-vs-gossip.pdf}
  \caption{Metric learning: comparison between our algorithm and an unbiased version}
  \label{fig:async_ml_baseline-vs-gossip}
\end{figure}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{.45\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{async_ml_cancer_standard}
    \caption{Evolution of the objective function and its standard deviation (asynchronous case).}
    \label{fig:async_ml_cancer_standard}
  \end{subfigure}
  \begin{subfigure}[t]{.45\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{async_ml_cancer_bias}
    \caption{Evolution of the bias term.}
    \label{fig:async_ml_cancer_bias}
  \end{subfigure}
  % \caption{Metric learning: evolution of the bias term $\overline{\epsilon}^n(t)^{\top}\omega(t)$.}
  \caption{Metric learning experiments on a real dataset.}
\end{figure*}

